Towards LLM-based optimization compilers. Can LLMs learn how to apply a single peephole optimization? Reasoning is all LLMs need!

Large Language Models (LLMs) have demonstrated great potential in various language processing tasks, and recent studies have explored their application in compiler optimizations. However, all these studies focus on the conventional open-source LLMs, such as Llama2, which lack enhanced reasoning mechanisms. In this study, we investigate the errors produced by the fine-tuned 7B-parameter Llama2 model as it attempts to learn and apply a simple peephole optimization for the AArch64 assembly code. We provide an analysis of the errors produced by the LLM and compare it with state-of-the-art OpenAI models which implement advanced reasoning logic, including GPT-4o and GPT-o1 (preview). We demonstrate that OpenAI GPT-o1, despite not being fine-tuned, outperforms the fine-tuned Llama2 and GPT-4o. Our findings indicate that this advantage is largely due to the chain-of-thought reasoning implemented in GPT-o1. We hope our work will inspire further research on using LLMs with enhanced reasoning mechanisms and chain-of-thought for code generation and optimization.

==> sections/background.tex <==
\section{Background}
\textbf{Compiler and ISA:} Peephole is an optimization technique applied at the basic block level that involves replacing the instructions with a logically equivalent set that has better performance \cite{Muchnick1997}. Peephole employs numerous pattern matching algorithms to apply a wide range of optimization scenarios. Its replacements include but are not limited to the following \cite{fischer2010crafting} :
\begin{itemize}
    \item Null sequences – Remove instructions which results are not used.
    \item Combine operations – Replace multiple operations with a single equivalent one.
    \item Algebraic optimizations – Apply algebraic laws to simplify or rearrange instructions.
    \item Address mode operations – Memory address algebraic optimizations.
    \item Special case instructions – Use of special instructions and operands, such as zero operand.
\end{itemize}

In our study, we train LLMs using the LLVM compiler and AArch64 instruction set architecture. LLVM contains two peephole implementations: \textit{InstructionCombining} \cite{LLVMInstructionCombining} and \textit{AArch64MIPeepholeOpt} \cite{LLVMAArch64MIPeepholeOpt}. The first implementation includes a large number of optimizations listed above, while the second seven specific matching methods for handling special optimizations in AArch64.


In LLVM, the source code goes through three parts: the Frontends, the Intermediate Representation(IR), and the Backends to generate instructions for the specified platform. For AArch64 instructions, peephole optimization occurs in the IR and the Backends machine instructions. These correspond to two optimization passes: \textit{InstructionCombining} \cite{LLVMInstructionCombining} and AArch64MIPeepholeOpt \cite{LLVMAArch64MIPeepholeOpt}.The former includes a large number of peephole optimization matching rules, which can be categorized into constant folding, strength reduction, null sequences, combine operations, algebraic laws, and address mode operations \cite{Bhatt2013}. The latter includes seven specific matching methods for handling special optimizations in AArch64. During optimization, the above methods are applied through multiple iterations. However, unlike these methods, LLM generates the final optimization results directly without iterative processing.

To cover a wider range of peephole optimization scenarios, we chose to provide the optimization results of InstructionCombining for the model to learn. TABLE I shows 6 categories of AArch64 instruction optimizations within our corpus as a result of InstructionCombining.



\begin{figure}[htbp]
\centering
\includegraphics[width=0.45\textwidth]{AArch64 structure.png}
\caption{AArch64 Structure}
\label{AArch64 structure}
\end{figure}



A typical AArch64 instruction set structure, as shown in Fig. \ref{AArch64 structure},  the file header, segment definitions, basic blocks and file footer \cite{ARM2024}. In compiler construction, a basic block is a straight-line code sequence with no branches in except to the entry and no branches out except at the exit \cite{Hennessy2011}\cite{Cooper2012}.

One of the characteristics of the InstructionCombining pass is that it does not alter the control flow graph (CFG) \cite{LLVMInstructionCombining} . Therefore, we exclude instructions that contain control flow and only process instructions that contain a single basic block, which also fits the peephole optimization requirement for a small window. At the same time, it reduces the window size of the large model.


\begin{figure*}[htbp]
\centering
\includegraphics[width=1\textwidth]{model_flow.png}
\caption{Model Flow}
\label{Model Flow}
\end{figure*}


\begin{table*}[htbp]
\renewcommand{\arraystretch}{1.2}
\caption{Categories of AArch64 Instruction Optimizations from InstructionCombining. The stack operations have been omitted from the non-optimized code except for the Address Mode Operation.}
\label{tab:}
\centering
\small
\begin{tabular}{p{0.2\textwidth} p{0.25\textwidth} p{0.2\textwidth} p{0.2\textwidth}}
\toprule
\textbf{Optimization Type} & \textbf{Non-optimized Code} & \textbf{Optimized Code} & \textbf{Description} \\
\midrule
\textbf{Constant Folding} & 
\begin{verbatim}
mov w0, #2
add w0, w0, #3
ret
\end{verbatim} &
\begin{verbatim}
mov w0, #5 
ret
\end{verbatim} &
The addition operation is folded into a single assignment. \\
\midrule
\textbf{Strength Reduction} & 
\begin{verbatim}
mov w1, w0 
mul w0, w1, #2 
ret
\end{verbatim} &
\begin{verbatim}
lsl w0, w0, #1
\end{verbatim} &
Multiplication by 2 is reduced to a left shift operation. \\
\midrule
\textbf{Null Sequences} & 
\begin{verbatim}
lsl w8, w8, #1
lsr w8, w8, #0
ret
\end{verbatim} &
\begin{verbatim}
lsl w0, w0, #1
ret
\end{verbatim} &
Right shift by 0 is effectively a no-op. \\
\midrule
\textbf{Combine Operations} & 
\begin{verbatim}
lsl x2, x1, #1      
add x3, x2, x2
\end{verbatim} &
\begin{verbatim}
add x3, x1, x1
\end{verbatim} &
Two expressions are combined into one. \\
\midrule
\textbf{Algebraic Laws} & 
\begin{verbatim}
mov w9, wzr
mul w8, w8, w9
ret
\end{verbatim} &
\begin{verbatim}
mov w0, wzr
ret
\end{verbatim} &
Any number multiplied by 0 is 0. \\
\midrule
\textbf{Address Mode Operations} & 
\begin{verbatim}
sub sp, sp, #16 
.cfi_def_cfa_offset 16
mov w8, #1 
str w8, [sp, #12] 
ldr w0, [sp, #12] 
add sp, sp, #16 
ret
\end{verbatim} &
\begin{verbatim} 
mov w0, #1
ret
\end{verbatim} &
Unnecessary stack read/write operations are eliminated. The addressing mode is optimized from indirect to immediate. \\
\bottomrule
\end{tabular}
\normalsize
\end{table*}

\begin{table}[htbp]
\renewcommand{\arraystretch}{1.2}
\caption{Examples demonstrating the LlaMa2 model's understanding of AArch64 instructions without fine-tuning. (a) and (b) show that LlaMa2 accurately interprets the instructions, while (c) illustrates a more complex case where LlaMa2 fails to correctly comprehend the instruction.}
\label{tab:LlaMa2_aarch64}
\normalsize
\begin{tabular}{p{8cm}}
\hline
\textbf{Prompt:} What does \texttt{ldr} mean in AArch64 instructions? \\
\textbf{Response:} The \texttt{ldr} instruction loads a 64-bit value from memory into a 64-bit register. \\
\textbf{(a)} This response is correct. \\
\hline
\textbf{Prompt:} What does \texttt{sub} mean in AArch64 instructions? \\
\textbf{Response:} A \texttt{sub} instruction in AArch64 is an instruction that performs a subtraction operation on two 64-bit operands. \\
\textbf{(b)} This response is correct. \\
\hline
\textbf{Prompt:} What does \texttt{.cfi\_def\_cfa\_offset} mean in AArch64 instructions? \\
\textbf{Response:} The \texttt{.cfi\_def\_cfa\_offset} instruction is used to define the CFA (Call Frame Address) register in AArch64 instructions. \\
\textbf{(c)} Incorrect. The \texttt{.cfi\_def\_cfa\_offset} instruction is used to define the offset of the Canonical Frame Address (CFA), not the CFA register itself. \\
\hline
\end{tabular}
\end{table}

\begin{figure}[htbp]
\centering
\begin{minipage}{0.48\linewidth}
\centering
\begin{lstlisting}[frame=single, basicstyle=\footnotesize\ttfamily, breaklines=true]
    // %bb.0:
    sub sp, sp, #16
    .cfi_def_cfa_offset 16
    mov w8, #2
    str w8, [sp, #12]
    ldr w8, [sp, #12]
    add w8, w8, #3
    str w8, [sp, #12]
    ldr w0, [sp, #12]
    add sp, sp, #16
    ret
\end{lstlisting}
\caption*{(a) Raw non-optimized instruction.}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
\centering
\begin{lstlisting}[frame=single, basicstyle=\footnotesize\ttfamily, breaklines=true]
    // %bb.0:
    sub sp, sp, #16
    .cfi_def_cfa_offset 16
    mov w8, #2
    str w8, [sp, #12]
    ldr w8, [sp, #12]
    add w8, w8, #3
    str w8, [sp, #12]
    ldr w0, [sp, #12]
    add sp, sp, #16
    ret
\end{lstlisting}
\caption*{(b) Instruction generated by the model.}
\end{minipage}

\vspace{1em}

\begin{minipage}{0.48\linewidth}
\centering
\begin{lstlisting}[frame=single, basicstyle=\footnotesize\ttfamily, breaklines=true]
    // %bb.0:
    mov w0, #5
    ret
\end{lstlisting}
\caption*{(c) Required optimized instruction.}
\end{minipage}

\caption{An example illustrating that a LlaMa2 model without fine-tuning is unable to perform peephole optimization on the AArch64 instructions.}

\label{fig:example}
\end{figure}
